A Free Knob: A Sensitivity Audit for Calibration in Threshold-based Evaluation

Many benchmarks for rare events score a prediction in three steps: pool the prediction and the target over spatial blocks, threshold each pooled field, and score the resulting contingency table. We show that at a fixed rare threshold the max-pooled Critical Success Index (CSI) cannot separate two different things: how well a system places events, and how well its amplitudes are calibrated. Sharp observations push many blocks above the threshold, while the attenuated predictions of squared-error regression leave those same blocks below it. A monotone calibration map is fitted on held-out data and applied separately to each system. The map needs no retraining and cannot change the order of any two pixels, so whatever part of a difference it reproduces cannot be evidence of better spatial ranking. We report how much of a reported difference the map removes. On SEVIR, two released checkpoints of one architecture differ by -29.5% in extreme-threshold CSI before the control and by +5.3% after it. Across 450 pairwise contrasts among 6 systems, how far apart two systems sit in pooled frequency bias predicts how far their CSI difference moves under the control (r = 0.896 when the map is fitted after pooling), and 64 contrasts reverse sign. At CasCast's published extreme-event operating point, calibration alone removes 88%-106% of the cascade's gain over its backbone across three controls. Calibration also reveals advantages hidden by a better-calibrated baseline. On geostationary infrared imagery, a larger share of the score can be explained by calibration as events get rarer. The problem therefore needs two things at the same time: a threshold that is fixed in advance, and a model whose output is poorly calibrated at that threshold. We recommend reporting pooled frequency bias and a symmetric held-out FreeKnob Audit alongside rare-event pool-and-threshold scores.

==> tab_atmos.tex <==
220 & 20.27\% & 0.2574 & 0.2679 & -0.0105 & 0/5 & -0.0086 \\
215 & 11.54\% & 0.1964 & 0.2056 & -0.0092 & 1/5 & -0.0121 \\
210 & 6.38\% & 0.1340 & 0.1460 & -0.0120 & 1/5 & -0.0177 \\
205 & 3.12\% & 0.0888 & 0.0842 & +0.0046 & 3/5 & +0.0023 \\
200 & 0.88\% & 0.0437 & 0.0445 & -0.0007 & 2/5 & -0.0005 \\
197 & 0.26\% & 0.0262 & 0.0360 & -0.0098 & 0/5 & -0.0086 \\


==> tab_crowd.tex <==
2.0 & 16.82\% & 0.4218 & 0.4684 & -0.0465 & 2/5 & 0.312 & -0.0813 \\
3.0 & 11.26\% & 0.4223 & 0.4466 & -0.0244 & 2/5 & 0.625 & -0.0286 \\
4.0 & 8.67\% & 0.4366 & 0.4428 & -0.0062 & 2/5 & 0.812 & -0.0329 \\
5.0 & 6.28\% & 0.3955 & 0.3910 & +0.0045 & 3/5 & 1.000 & -0.0421 \\
7.0 & 3.77\% & 0.3553 & 0.3207 & +0.0346 & 5/5 & 0.062 & -0.0489 \\
10.0 & 2.50\% & 0.3038 & 0.2841 & +0.0197 & 4/5 & 0.312 & -0.0743 \\
15.0 & 1.82\% & 0.3541 & 0.2968 & +0.0574 & 5/5 & 0.062 & -0.1495 \\


==> tab_dose.tex <==
persistence (a real radar field) & 0.999 & 1.004 & 1.020 & -0.3\% & +0.0\% & -0.8\% \\
pysteps LK (advection) & 0.910 & 0.918 & 0.907 & +0.7\% & +0.4\% & +0.2\% \\
EarthFormer & 0.534 & 0.337 & 0.281 & +5.0\% & +22.2\% & +20.3\% \\
CasCast backbone & 0.495 & 0.285 & 0.172 & +11.8\% & +42.4\% & +79.8\% \\
CasCast cascade & 0.905 & 0.904 & 1.037 & -1.1\% & -1.0\% & -2.9\% \\


==> tab_radar.tex <==
0.1mm & 0.7543 & 0.7543 & 0.7553 & -0.0009 & -0.0009 \\
0.5mm & 0.5899 & 0.5897 & 0.5873 & +0.0026 & +0.0025 \\
1mm & 0.3891 & 0.4595 & 0.4532 & -0.0640 & +0.0063 \\
2.5mm & 0.3354 & 0.3435 & 0.3440 & -0.0087 & -0.0005 \\
5mm & 0.2058 & 0.2034 & 0.2110 & -0.0052 & -0.0076 \\


==> tab_samearch_exact.tex <==
16 & 0.915 & 0.875 & -0.0109 & +0.0006 & -1.4\% & +0.1\% \\
74 & 0.747 & 0.718 & -0.0150 & +0.0005 & -2.2\% & +0.1\% \\
133 & 0.535 & 0.495 & -0.0238 & +0.0013 & -5.1\% & +0.2\% \\
160 & 0.387 & 0.337 & -0.0315 & +0.0014 & -9.5\% & +0.3\% \\
181 & 0.336 & 0.285 & -0.0323 & +0.0047 & -11.3\% & +1.2\% \\
219 & 0.280 & 0.172 & -0.0614 & +0.0089 & -29.5\% & +2.8\% \\


==> tab_samearch_exact_ci.tex <==
16 & 0.91 / 0.87 & -0.0109 [-0.0125, -0.0094] & +0.0006 [-0.0003, +0.0014] \\
74 & 0.75 / 0.72 & -0.0150 [-0.0171, -0.0129] & +0.0005 [-0.0007, +0.0018] \\
133 & 0.53 / 0.49 & -0.0238 [-0.0272, -0.0202] & +0.0013 [-0.0004, +0.0031] \\
160 & 0.39 / 0.34 & -0.0315 [-0.0358, -0.0274] & +0.0014 [-0.0010, +0.0040] \\
181 & 0.34 / 0.28 & -0.0323 [-0.0371, -0.0280] & +0.0047 [+0.0013, +0.0079] \\
219 & 0.28 / 0.17 & -0.0614 [-0.0695, -0.0536] & +0.0089 [+0.0044, +0.0136] \\

